Statistical Analysis of Complex Computer Models in Astronomy

We introduce statistical techniques required to handle complex computer models with potential applications to astronomy. Computer experiments play a critical role in almost all fields of scientific research and engineering. These computer experiments, or simulators, are often computationally expensive, leading to the use of emulators for rapidly approximating the outcome of the experiment. Gaussian process models, also known as Kriging, are the most common choice of emulator. While emulators offer significant improvements in computation over computer simulators, they require a selection of inputs along with the corresponding outputs of the computer experiment to function well. Thus, it is important to select inputs judiciously for the full computer simulation to construct an accurate emulator. Space-filling designs are efficient when the general response surface of the outcome is unknown, and thus they are a popular choice when selecting simulator inputs for building an emulator. In this tutorial we discuss how to construct these space filling designs, perform the subsequent fitting of the Gaussian process surrogates, and briefly indicate their potential applications to astronomy research.

==> submission_text.tex <==
Dear Editor,

Please find enclosed the manuscript “Statistical Analysis of Complex Computer Models in Astronomy” by Lukemire et al., which we ask you to consider for publication in EPJST.

Our manuscript provides a tutorial to astronomy researchers concerning the use of surrogate models to work with complex computer experiments. This is an important and highly relevant research area. We believe the astronomy community is less familiar with the statistical aspects concerning the experimental design, especially using metaheuristic algorithms. These metaheuristic approaches are well-known in the astronomy community for analysing experiments, but to the best of our knowledge have not been frequently used in the context of obtaining an optimal set of inputs for computer experiments with the intent of constructing an emulator or surrogate model. Throughout our manuscript we illustrate the discussed approaches using statistical software.

We hope that you will like our manuscript and find it suitable for publication in EPJST.

Thanks,

Abhyuday Mandal
